Slither: A Static Analysis Framework For Smart Contracts

This paper describes Slither, a static analysis framework designed to provide rich information about Ethereum smart contracts. It works by converting Solidity smart contracts into an intermediate representation called SlithIR. SlithIR uses Static Single Assignment (SSA) form and a reduced instruction set to ease implementation of analyses while preserving semantic information that would be lost in transforming Solidity to bytecode. Slither allows for the application of commonly used program analysis techniques like dataflow and taint tracking. Our framework has four main use cases: (1) automated detection of vulnerabilities, (2) automated detection of code optimization opportunities, (3) improvement of the user's understanding of the contracts, and (4) assistance with code review. In this paper, we present an overview of Slither, detail the design of its intermediate representation, and evaluate its capabilities on real-world contracts. We show that Slither's bug detection is fast, accurate, and outperforms other static analysis tools at finding issues in Ethereum smart contracts in terms of speed, robustness, and balance of detection and false positives. We compared tools using a large dataset of smart contracts and manually reviewed results for 1000 of the most used contracts.

==> slithir_instructions_tables.tex <==
\begin{table}
\begin{centering}
\subfloat[ \label{subtable:slithir1} ]{%
\begin{tabular}{|l|l|}
\hline 
Type & Instruction\tabularnewline
\hline 
\hline 
\multirow{3}{*}{Assignement} & $\text{LV}\coloneqq\text{RV}$\tabularnewline
\cline{2-2} 
 & $\text{LV}\coloneqq(\text{RV}_{1},\text{RV}_{2})$ \tabularnewline
\cline{2-2} 
 & $\text{LV}\coloneqq\text{FUN}$\tabularnewline
\hline 
\multirow{19}{*}{Binary Operation} & $\text{LV}=\text{RV}_{1}**\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}*\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}/\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\%\text{RV}_{1}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}+\text{RV}_{1}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}-\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\ll\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\gg\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\text{\&}\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\wedge\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}|\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}<\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}>\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\leq\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\geq\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}==\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}!=\text{RV}_{2}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}\&\&\text{RV}_{2}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{RV}_{1}--\text{RV}_{2}$ \tabularnewline
\hline 
\multirow{3}{*}{Unary Operation} & $\text{LV}=\text{!RV}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{\textasciitilde RV}$\tabularnewline
\cline{2-2} 
 & $\text{DELETE LV}$\tabularnewline
\hline 
Index & $\text{REF}\rightarrow\text{LV [RV] }$ \tabularnewline
\hline 
\end{tabular}

}\subfloat[ \label{subtable:slithir2} ]{%
\begin{tabular}{|l|l|}
\hline 
Type & Instruction\tabularnewline
\hline 
\hline 
\multirow{3}{*}{Member} & $\text{REF}\rightarrow\text{LV . RV }$ \tabularnewline
\cline{2-2} 
 & $\text{REF}\rightarrow\text{CONTRACT . RV }$\tabularnewline
\cline{2-2} 
 & $\text{REF}\rightarrow\text{ENUM . RV }$\tabularnewline
\hline 
\multirow{4}{*}{New Operators} & $\text{LV}=\text{NCONTRACT CONST}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{NSTRUCTURE STRUC}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{NETYPE TYPE}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{NARRAY ARRAY\_TYPE DEPTH}$ \tabularnewline
\hline 
\multirow{2}{*}{Push Operands} & $\text{PUSH LV}$RV \tabularnewline
\cline{2-2} 
 & $\text{PUSH LV}$FUN \tabularnewline
\hline 
Conversion & $\text{CONVERT LV RV TYPE}$\tabularnewline
\hline 
Unpack & $\text{LV}=\text{UNPACK TUPLE INDEX}$\tabularnewline
\hline 
Array Initialization  & $\text{LV}=\text{INIT\_VALUES}$\tabularnewline
\hline 
\multirow{9}{*}{Calls Operators} & $\text{LV}=\text{HCALL DEST FUN [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{LCALL DEST FUN [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{SCALL FUN [ARG, ..]}$ \tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{ICALL FUN [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{IDCALL FUN\_TYPE [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{LCALL DEST FUN [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{ECALL EVENT [ARG, ..]}$\tabularnewline
\cline{2-2} 
 & $\text{LV}=\text{SEND DEST VALUE}$\tabularnewline
\cline{2-2} 
 & $\text{TRANSFER DEST VALUE}$ \tabularnewline
\hline 
\multirow{3}{*}{Return} & $\text{RETURN RV}$ \tabularnewline
\cline{2-2} 
 & $\text{RETURN TUPLE}$\tabularnewline
\cline{2-2} 
 & $\text{RETURN NONE}$ \tabularnewline
\hline 
Condition & $\text{CONDITION RV}$ \tabularnewline
\hline 
\end{tabular}

}
\par\end{centering}
\caption{Part of SlithIR instruction set}

\end{table}

